Using Large Language Models to Develop Requirements Elicitation Skills

Requirements Elicitation (RE) is a crucial software engineering skill that involves interviewing a client and then devising a software design based on the interview results. Teaching this inherently experiential skill effectively has high cost, such as acquiring an industry partner to interview, or training course staff or other students to play the role of a client. As a result, a typical instructional approach is to provide students with transcripts of real or fictitious interviews to analyze, which exercises the skill of extracting technical requirements but fails to develop the equally important interview skill itself. As an alternative, we propose conditioning a large language model to play the role of the client during a chat-based interview. We perform a between-subjects study (n=120) in which students construct a high-level application design from either an interactive LLM-backed interview session or an existing interview transcript describing the same business processes. We evaluate our approach using both a qualitative survey and quantitative observations about participants' work. We find that both approaches provide sufficient information for participants to construct technically sound solutions and require comparable time on task, but the LLM-based approach is preferred by most participants. Importantly, we observe that LLM-backed interview is seen as both more realistic and more engaging, despite the LLM occasionally providing imprecise or contradictory information. These results, combined with the wide accessibility of LLMs, suggest a new way to practice critical RE skills in a scalable and realistic manner without the overhead of arranging live interviews.

==> Makefile <==

#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PAPER=cleia

all: $(PAPER).pdf TAGS

zip: clean
	cd .. && zip -r iticse195.zip $(shell basename $(CURDIR)) -x '$(shell basename $(CURDIR))/.git/*' -x .gitignore -x TAGS

$(PAPER).pdf: $(wildcard *.tex) $(wildcard figs/*) $(wildcard *.bib)
	pdflatex $(PAPER)
	- bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $(PAPER); done

.PHONY: clean
clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	$(PAPER).pdf

TAGS: $(wildcard *.tex) $(wildcard figs/*) $(wildcard *.bib)
	- etags $^



==> authors-anon.tex <==
\author{Anon Author 1}\email{anon@anon.net}
\affiliation{%
    \institution{Anon Institution}
%  \city{Anon City}
%  \state{Anon State}
  \country{Anon Country}
}

\author{Anon Author 2}\email{anon@anon.net}
\orcid{0000-0000-0000-0000}
\affiliation{%
    \institution{Anon Institution}
%  \city{Anon City}
%  \state{Anon State}
  \country{Anon Country}
}
\author{Anon Author 3}\email{anon@anon.net}
\orcid{0000-0000-0000-0000}
\affiliation{%
    \institution{Anon Institution}
%  \city{Anon City}
%  \state{Anon State}
  \country{Anon Country}
}
\author{Anon Author 4}\email{anon@anon.net}
\orcid{0000-0000-0000-0000}
\affiliation{%
    \institution{Anon Institution}
%  \city{Anon City}
%  \state{Anon State}
  \country{Anon Country}
}
\author{Anon Author 5}\email{anon@anon.net}
\orcid{0000-0000-0000-0000}
\affiliation{%
    \institution{Anon Institution}
%  \city{Anon City}
%  \state{Anon State}
  \country{Anon Country}
}
\author{Anon Author 6}\email{anon@anon.net}
\orcid{0000-0000-0000-0000}
\affiliation{%
    \institution{Anon Institution}
%  \city{Anon City}
%  \state{Anon State}
  \country{Anon Country}
}
\author{Anon Author 7}\email{anon@anon.net}
\orcid{0000-0000-0000-0000}
\affiliation{%
    \institution{Anon Institution}
%  \city{Anon City}
%  \state{Anon State}
  \country{Anon Country}
}

==> questions-table.tex <==
\begin{table}
    \centering
    \begin{tabular}{p{0.3cm}p{7.2cm}}
\hline
%\textbf{ID} & \textbf{Question} \\
%\hline
%\multicolumn{2}{p{7.5cm}}{\textbf{Regarding the exercise:}} \\
%\hline
Q1 & The time provided to solve the exercise was sufficient \\
\hline
Q2 & The difficulty of the exercise was appropriate \\
\hline
Q3 & The solution provided by the instructors for evaluating the exercise  made sense \\
\hline
Q4 & The evaluation of my solution (compared with the solution provided by instructors) was appropriate \\
\hline
%\multicolumn{2}{p{7.5cm}}{\textbf{Regarding the C-LEIA behavior:} (these questions given to EG only)} \\
\hline
Q5* & (EG only) The C-LEIA provided enough information to solve the design problem \\
\hline
Q6* & (EG only) The C-LEIA provided useful information \\ %
\hline
Q7* & (EG only) The C-LEIA avoided technical jargon (regarding software engineering and development) in its responses \\
\hline
%\multicolumn{2}{p{7.5cm}}{\textbf{Regarding the usefulness of the C-LEIA in improving your interviewing skills and RE skills:} (these questions given to EG only)} \\
\hline
Q8* & The interaction with the C-LEIA helped me to improve as an active listener---understanding both what is said and what is unsaid, identifying the nuances and underlying concerns that may not be immediately apparent. \\
\hline
Q9* & The interaction with the C-LEIA improved my ability to communicate clearly and ask more accurate and precise questions. \\
\hline
Q10* & Interacting with the C-LEIA could help me improve in asking open-ended questions, which are essential for encouraging expansive responses and uncovering missing client needs/requirements. \\
\hline
Q11* & Through interaction with the C-LEIA, I could enhance my ability to ask closed-ended questions, which are crucial for clarifying specific points and ensuring accuracy in understanding client requirements. \\
\hline
Q12* & Interacting with the C-LEIA could help me improve in identifying and managing different stakeholders, each with their own needs, priorities, and influence on the project. \\
%\hline
\hline
%\multicolumn{2}{p{7.5cm}}{\textbf{During the exercise:}} \\
\hline
Q13 & I felt engaged with the task \\
\hline
Q14 & The interaction with the tool used for gathering requirements (C-LEIA or Transcript) was motivating \\
\hline
Q15 & The tool used to elicit requirements information kept me interested in the activity \\
\hline
\end{tabular}
\caption{Likert scale survey questions (*=optional). The form also solicited free-text comments. Q5--Q11 were only given to the experimental group.  Q15--Q16 were answered by the control group with respect to the transcript and by the experimental group with respect to the C-LEIA session.}
\label{tab:survey_questions}
\end{table}

